Band structure and giant Stark effect in two-dimensional transition-metal dichalcogenides

We present a comprehensive study of the electronic structures of 192 configurations of 39 stable, layered, transition-metal dichalcogenides using density-functional theory. We show detailed investigations of their monolayer, bilayer, and trilayer structures' valence-band maxima, conduction-band minima, and band gap responses to transverse electric fields. We also report the critical fields where semiconductor-to-metal phase transitions occur. Our results show that band gap engineering by applying electric fields can be an effective strategy to modulate the electronic properties of transition-metal dichalcogenides for next-generation device applications.

==> TMDCRef.tex <==
@article {Hsien2012,
author = {Lee, Yi-Hsien and Zhang, Xin-Quan and Zhang, Wenjing and Chang, Mu-Tung and Lin, Cheng-Te and Chang, Kai-Di and Yu, Ya-Chu and Wang, Jacob Tse-Wei and Chang, Chia-Seng and Li, Lain-Jong and Lin, Tsung-Wu},
title = {Synthesis of Large-Area MoS2 Atomic Layers with Chemical Vapor Deposition},
journal = {Adv. Mater.},
volume = {24},
number = {17},
publisher = {WILEY-VCH Verlag},
issn = {1521-4095},
doi = {10.1002/adma.201104798},
pages = {2320-2325},
month={March},
year = {2012},
}

@Article{Shaw2014,
author="Shaw, Jonathan C.
and Zhou, Hailong
and Chen, Yu
and Weiss, Nathan O.
and Liu, Yuan
and Huang, Yu
and Duan, Xiangfeng",
title="Chemical vapor deposition growth of monolayer MoSe2 nanosheets",
journal="Nano Res.",
year="2014",
month="Apr",
day="01",
volume="7",
number="4",
pages="511-517",
month={January},
issn="1998-0000",
doi="10.1007/s12274-014-0417-z",
}

@article{Zhang2013,
author = {Zhang, Yu and Zhang, Yanfeng and Ji, Qingqing and Ju, Jing and Yuan, Hongtao and Shi, Jianping and Gao, Teng and Ma, Donglin and Liu, Mengxi and Chen, Yubin and Song, Xiuju and Hwang, Harold Y. and Cui, Yi and Liu, Zhongfan},
title = {Controlled Growth of High-Quality Monolayer WS2 Layers on Sapphire and Imaging Its Grain Boundary},
journal = {ACS Nano},
volume = {7},
month={September},
number = {10},
pages = {8963-8971},
year = {2013},
doi = {10.1021/nn403454e},

}

@article{Kang2013,
author = {Kang, Kibum and Xie, Saien and Huang, Lujie and Han, Yimo and Huang, Pinshane Y. and Mak, Kin Fai and Kim, Cheol-Joo and Muller, David and Park, Jiwoong},
title = {High-mobility three-atom-thick semiconducting films with wafer-scale homogeneity},
journal = {Nature},
volume = {520},
month={April},
number = {7549},
pages = {656-660},
year = {2015},
url = {http://dx.doi.org/10.1038/nature14417},

}





@article{Miguel,
author = {Ugeda, Miguel M. and Bradley, Aaron J. and Zhang, Yi and Onishi, Seita and Chen, Yi and Ruan, Wei and Ojeda-Aristizabal, Claudia and Ryu, Hyejin and Edmonds, Mark T. and Tsai, Hsin-Zon and Riss, Alexander and Mo, Sung-Kwan and Lee, Dunghai and Zettl, Alex and Hussain, Zahid and Shen, Zhi-Xun and Crommie, Michael F.},

title = {Characterization of collective ground states in single-layer NbSe2},
journal = {Nat. Phys.},
volume = {12},
month={January},
number = {1},
pages = {92-97},
year = {2016},
Publisher={Nature Publishing Group},
url = {http://dx.doi.org/10.1038/nphys3527},
}


@article{Miguel2014,
author = {Ugeda, Miguel M. and Bradley, Aaron J. and Shi, Su-Fei and da Jornada, Felipe H. and Zhang, Yi and Qiu, Diana Y. and Ruan, Wei and Mo, Sung-Kwan and Hussain, Zahid and Shen, Zhi-Xun and Wang, Feng and Louie, Steven G. and Crommie, Michael F..},

title = {Giant bandgap renormalization and excitonic effects in a monolayer transition metal dichalcogenide semiconductor},
journal = {Nat. Mater.},
volume = {13},
number = {12},
pages = {1091-1095},
year = {2014},
month={December},
Publisher={Nature Publishing Group},
url = {http://dx.doi.org/10.1038/nmat4061},
}

@article{Barja2016,
author = {Barja, Sara and Wickenburg, Sebastian and Liu, Zhen-Fei and Zhang, Yi and Ryu, Hyejin and Ugeda, Miguel M. and Hussain, Zahid and Shen, Zhi-Xun and Mo, Sung-Kwan and Wong, Ed and Salmeron, Miquel B. and Wang, Feng and Crommie, Michael F. and Ogletree, D. Frank and Neaton, Jeffrey B. and Weber-Bargioni, Alexander},

title = {Charge density wave order in 1D mirror twin boundaries of single-layer MoSe2},
journal = {Nat. Phys.},
volume = {12},
number = {8},
pages = {751-756},
year = {2016},
month={DAugust},
Publisher={Nature Publishing Group},
url = {http://dx.doi.org/10.1038/nphys3730},
}

@article{Dumceno,
author = {Dumcenco, Dumitru and Ovchinnikov, Dmitry and Marinov, Kolyo and Lazić, Predrag and Gibertini, Marco and Marzari, Nicola and Sanchez, Oriol Lopez and Kung, Yen-Cheng and Krasnozhon, Daria and Chen, Ming-Wei and Bertolazzi, Simone and Gillet, Philippe and Fontcuberta i Morral, Anna and Radenovic, Aleksandra and Kis, Andras},
title = {Large-Area Epitaxial Monolayer MoS2},
journal = {ACS Nano},
volume = {9},
number = {4},
month={April},
pages = {4611-4620},
year = {2015},
doi = {10.1021/acsnano.5b01281},
URL = { 
        http://dx.doi.org/10.1021/acsnano.5b01281   
}
}

@article{Xingli,
author = {Wang, Xingli and Gong, Yongji and Shi, Gang and Chow, Wai Leong and Keyshar, Kunttal and Ye, Gonglan and Vajtai, Robert and Lou, Jun and Liu, Zheng and Ringe, Emilie and Tay, Beng Kang and Ajayan, Pulickel M.},
title = {Chemical Vapor Deposition Growth of Crystalline Monolayer MoSe2},
journal = {ACS Nano},
volume = {8},
number = {5},
month={March},
pages = {5125-5131},
year = {2014},
doi = {10.1021/nn501175k},
URL = { 
        http://dx.doi.org/10.1021/nn501175k 
},

}

@article{Chang2014,
author = {Chang, Yung-Huang and Zhang, Wenjing and Zhu, Yihan and Han, Yu and Pu, Jiang and Chang, Jan-Kai and Hsu, Wei-Ting and Huang, Jing-Kai and Hsu, Chang-Lung and Chiu, Ming-Hui and Takenobu, Taishi and Li, Henan and Wu, Chih-I and Chang, Wen-Hao and Wee, Andrew Thye Shen and Li, Lain-Jong},
title = {Monolayer MoSe2 Grown by Chemical Vapor Deposition for Fast Photodetection},
journal = {ACS Nano},
volume = {8},
number = {8},
month={August},
pages = {8582-8590},
year = {2014},
doi = {10.1021/nn503287m},

}

@article {Chen2015,
author = {Chen, Jianyi and Liu, Bo and Liu, Yanpeng and Tang, Wei and Nai, Chang Tai and Li, Linjun and Zheng, Jian and Gao, Libo and Zheng, Yi and Shin, Hyun Suk and Jeong, Hu Young and Loh, Kian Ping},
title = {Chemical Vapor Deposition of Large-Sized Hexagonal WSe2 Crystals on Dielectric Substrates},
journal = {Adv. Mater.},
volume = {27},
number = {42},
issn = {1521-4095},
doi = {10.1002/adma.201503446},
pages = {6722-6727},
month={September},
year={2015}
}

@article{Yoshida2016,
author = {Yoshida, Masaro and Iizuka, Takahiko and Saito, Yu and Onga, Masaru and Suzuki, Ryuji and Zhang, Yijin and Iwasa, Yoshihiro and Shimizu, Sunao},
title = {Gate-Optimized Thermoelectric Power Factor in Ultrathin WSe2 Single Crystals},
journal = {Nano Lett.},
volume = {16},
number = {3},
month={February},
pages = {2061-2065},
year = {2016},
doi = {10.1021/acs.nanolett.6b00075},

}
@article{CHUNG1998137,
title = "WS2 thin films by metal organic chemical vapor deposition",
journal = "J. Cryst. Growth",
volume = "186",
number = "1",
pages = "137-150",
month="March",
year = "1998",
issn = "0022-0248",
doi = "http://dx.doi.org/10.1016/S0022-0248(97)00479-X",
author = "J.-W. Chung and Z.R. Dai and F.S. Ohuchi",
}
@article {Keyshar2015,
author = {Keyshar, Kunttal and Gong, Yongji and Ye, Gonglan and Brunetto, Gustavo and Zhou, Wu and Cole, Daniel P. and Hackenberg, Ken and He, Yongmin and Machado, Leonardo and Kabbani, Mohamad and Hart, Amelia H. C. and Li, Bo and Galvao, Douglas S. and George, Antony and Vajtai, Robert and Tiwary, Chandra Sekhar and Ajayan, Pulickel M.},
title = {Chemical Vapor Deposition of Monolayer Rhenium Disulfide (ReS2)},
journal = {Adv. Mater.},
volume = {27},
number = {31},
issn = {1521-4095},
doi = {10.1002/adma.201501795},
pages = {4640-4648},
month={July},
year = {2015},
}


@article {Hafeez2016,
author = {Hafeez, Muhammad and Gan, Lin and Li, Huiqiao and Ma, Ying and Zhai, Tianyou},
title = {Large-Area Bilayer ReS2 Film/Multilayer ReS2 Flakes Synthesized by Chemical Vapor Deposition for High Performance Photodetectors},
journal = {Adv. Funct. Mater.},
volume = {26},
number = {25},
issn = {1616-3028},
url = {http://dx.doi.org/10.1002/adfm.201601019},
doi = {10.1002/adfm.201601019},
pages = {4551-4560},
month={April},
year = {2016},
}

@article{Naylor2016,
author = {Naylor, Carl H. and Parkin, William M. and Ping, Jinglei and Gao, Zhaoli and Zhou, Yu Ren and Kim, Youngkuk and Streller, Frank and Carpick, Robert W. and Rappe, Andrew M. and Drndi\'{c}, Marija and Kikkawa, James M. and Johnson, A. T. Charlie},
title = {Monolayer Single-Crystal 1T$\prime$-MoTe2 Grown by Chemical Vapor Deposition Exhibits Weak Antilocalization Effect},
journal = {Nano Lett.},
volume = {16},
number = {7},
pages = {4297-4304},
year = {2016},
month={May},
doi = {10.1021/acs.nanolett.6b01342},
}

@article {Zhou2017,
author = {Zhou, Jiadong and Liu, Fucai and Lin, Junhao and Huang, Xiangwei and Xia, Juan and Zhang, Bowei and Zeng, Qingsheng and Wang, Hong and Zhu, Chao and Niu, Lin and Wang, Xuewen and Fu, Wei and Yu, Peng and Chang, Tay-Rong and Hsu, Chuang-Han and Wu, Di and Jeng, Horng-Tay and Huang, Yizhong and Lin, Hsin and Shen, Zexiang and Yang, Changli and Lu, Li and Suenaga, Kazu and Zhou, Wu and Pantelides, Sokrates T. and Liu, Guangtong and Liu, Zheng},
title = {Large-Area and High-Quality 2D Transition Metal Telluride},
journal = {Adv. Mater.},
volume = {29},
number = {3},
issn = {1521-4095},
month={November},
url = {http://dx.doi.org/10.1002/adma.201603471},
doi = {10.1002/adma.201603471},
pages = {1603471 (1-8)},
year = {2017},
}

@article{Dumitru,
  author={Dumitru Dumcenco and Dmitry Ovchinnikov and Oriol Lopez Sanchez and Philippe Gillet and Duncan T L Alexander and Sorin
Lazar and Aleksandra Radenovic and Andras Kis},
  title={Large-area MoS2 grown using H2S as the sulphur source},
  journal={2D Mater.},
  volume={2},
  number={4},
  pages={044005 (1-7)},
  month={November},
  url={http://stacks.iop.org/2053-1583/2/i=4/a=044005},
  year={2015},
}


@article{Eichfeld,
author = {Eichfeld, Sarah M. and Hossain, Lorraine and Lin, Yu-Chuan and Piasecki, Aleksander F. and Kupp, Benjamin and Birdwell, A. Glen and Burke, Robert A. and Lu, Ning and Peng, Xin and Li, Jie and Azcatl, Angelica and McDonnell, Stephen and Wallace, Robert M. and Kim, Moon J. and Mayer, Theresa S. and Redwing, Joan M. and Robinson, Joshua A.},
title = {Highly Scalable, Atomically Thin WSe2 Grown via Metal–Organic Chemical Vapor Deposition},
journal = {ACS Nano},
volume = {9},
number = {2},
pages = {2080-2087},
year = {2015},
month={January},
doi = {10.1021/nn5073286},
}


@article {Gao2015,
author = {Gao, Yang and Liu, Zhibo and Sun, Dong-Ming and Huang, Le and Ma, Lai-Peng and Yin, Li-Chang and Ma, Teng and Zhang, Zhiyong and Ma, Xiu-Liang and Peng, Lian-Mao and Cheng, Hui-Ming and Ren, Wencai},
title = {Chemical Vapor Deposition of Large-Sized Hexagonal WSe2 Crystals on Dielectric Substrates},
journal = {Nat. Commun.},
volume = {6},
url = {http://dx.doi.org/10.1038/ncomms9569},
pages = {8569 (1-10)},
month={October},
year={2015}
}

@article {Coleman568,
	author = {Coleman, Jonathan N. and Lotya, Mustafa and O{\textquoteright}Neill, Arlene and Bergin, Shane D. and King, Paul J. and Khan, Umar and Young, Karen and Gaucher, Alexandre and De, Sukanta and Smith, Ronan J. and Shvets, Igor V. and Arora, Sunil K. and Stanton, George and Kim, Hye-Young and Lee, Kangho and Kim, Gyu Tae and Duesberg, Georg S. and Hallam, Toby and Boland, John J. and Wang, Jing Jing and Donegan, John F. and Grunlan, Jaime C. and Moriarty, Gregory and Shmeliov, Aleksey and Nicholls, Rebecca J. and Perkins, James M. and Grieveson, Eleanor M. and Theuwissen, Koenraad and McComb, David W. and Nellist, Peter D. and Nicolosi, Valeria},
	title = {Two-Dimensional Nanosheets Produced by Liquid Exfoliation of Layered Materials},
	volume = {331},
	number = {6017},
	pages = {568-571},
	year = {2011},
	month={February},
	doi = {10.1126/science.1194975},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/331/6017/568},
	journal = {Science}
}

@article {Zeng2011,
author = {Zeng, Zhiyuan and Yin, Zongyou and Huang, Xiao and Li, Hai and He, Qiyuan and Lu, Gang and Boey, Freddy and Zhang, Hua},
title = {Single-Layer Semiconducting Nanosheets: High-Yield Preparation and Device Fabrication},
journal = {Angew. Chem. Int. Ed.},
volume = {50},
number = {47},
publisher = {WILEY-VCH Verlag},
issn = {1521-3773},
month={October},
doi = {10.1002/anie.201106004},
pages = {11093-11097},
}

@article {Zhan,
author = {Zhan, Yongjie and Liu, Zheng and Najmaei, Sina and Ajayan, Pulickel M. and Lou, Jun},
title = {Large-Area Vapor-Phase Growth and Characterization of MoS2 Atomic Layers on a SiO2 Substrate},
journal = {Small},
volume = {8},
number = {7},
month={February},
publisher = {WILEY-VCH Verlag},
issn = {1613-6829},
doi = {10.1002/smll.201102654},
pages = {966-971},
}


@Article{C2NR31833D,
author ="Lin, Yu-Chuan and Zhang, Wenjing and Huang, Jing-Kai and Liu, Keng-Ku and Lee, Yi-Hsien and Liang, Chi-Te and Chu, Chih-Wei and Li, Lain-Jong",
title  ="Wafer-scale MoS2 thin layers prepared by MoO3 sulfurization",
journal  ="Nanoscale",
year  ="2012",
volume  ="4",
month={August},
issue  ="20",
pages  ="6637-6641",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C2NR31833D",
}

@article{ENNAOUI1995124,
title = "Preparation of textured and photoactive 2H-WS2 thin films by sulfurization of WO3",
journal = "Thin Solid Films",
volume = "261",
number = "1",
pages = "124-131",
year = "1995",
month={June},
issn = "0040-6090",
doi = "http://dx.doi.org/10.1016/S0040-6090(95)06524-5",
url = "http://www.sciencedirect.com/science/article/pii/S0040609095065245",
author = "A. Ennaoui and S. Fiechter and K. Ellmer and R. Scheer and K. Diesner",
}




 @article{RT2015,
author = {Rasmussen, Filip A. and Thygesen, Kristian S.},
title = {Computational 2D Materials Database: Electronic Structure of Transition-Metal Dichalcogenides and Oxides},
journal = {J. Phys. Chem. C},
volume = {119},
number = {23},
pages = {13169},
year = {2015},
doi = {10.1021/acs.jpcc.5b02950},
}

@article{PRL105,
  title = {Atomically Thin ${\mathrm{MoS}}_{2}$: A New Direct-Gap Semiconductor},
  author = {Mak, Kin Fai and Lee, Changgu and Hone, James and Shan, Jie and Heinz, Tony F.},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {13},
  pages = {136805},
  numpages = {4},
  year = {2010},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.136805},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.105.136805}
}

@article{MoWS2,
  title = {Influence of quantum confinement on the electronic structure of the transition metal sulfide $T$S${}_{2}$},
  author = {Kuc, A. and Zibouche, N. and Heine, T.},
  journal = {Phys. Rev. B},
  volume = {83},
  issue = {24},
  pages = {245213},
  numpages = {4},
  year = {2011},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.83.245213},
}

@article{EmergingPL,
author = {Splendiani, Andrea and Sun, Liang and Zhang, Yuanbo and Li, Tianshu and Kim, Jonghwan and Chim, Chi-Yung and Galli, Giulia and Wang, Feng},
title = {Emerging Photoluminescence in Monolayer MoS2},
journal = {Nano Lett.},
volume = {10},
number = {4},
pages = {1271},
year = {2010},
doi = {10.1021/nl903868w},
}

@article{RNT2011,
  title = {Tunable band gaps in bilayer transition-metal dichalcogenides},
  author = {Ramasubramaniam, Ashwin and Naveh, Doron and Towe, Elias},
  journal = {Phys. Rev. B},
  volume = {84},
  issue = {20},
  pages = {205325},
  numpages = {10},
  year = {2011},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.84.205325},
}


@article{LLGC2012,
author = {Liu, Qihang and Li, Linze and Li, Yafei and Gao, Zhengxiang and Chen, Zhongfang and Lu, Jing},
title = {Tuning Electronic Structure of Bilayer MoS2 by Vertical Electric Field: A First-Principles Investigation},
journal = {J. Phys. Chem. C},
volume = {116},
number = {40},
pages = {21556-21562},
year = {2012},
doi = {10.1021/jp307124d},
}


@Article{Nguyen2016,
author="Nguyen, Chuong V.
and Hieu, Nguyen N.
and Ilyasov, Victor V.",
title="Band Gap Modulation of Bilayer MoS2 Under Strain Engineering and Electric Field: A Density Functional Theory",
journal="J. Electron. Mater.",
year="2016",
volume="45",
number="8",
pages="4038",

issn="1543-186X",
doi="10.1007/s11664-016-4593-3",
}

@article{SOC_MLS,
  title = {Spin-orbital effects in metal-dichalcogenide semiconducting monolayers},
  author = {Reyes-Retana, J. A. and Cervantes-Sodi, F.},
  journal = {Sci. Rep.},
  volume = {6},
  pages = {24093},
 year = {2016},
  month = {04},
  publisher = {The Author(s) SN},
}

@article{MoS2_ML_EF,
title = "Band structure modulation in MoS2 multilayers and heterostructures through electric field and strain ",
journal = "Comput. Mater. Sci.",
volume = "112, Part A",
number = "",
pages = "377",
year = "2016",
issn = "0927-0256",
doi = "http://dx.doi.org/10.1016/j.commatsci.2015.11.007",
author = "Nicholas A. Lanzillo and Terrance P. O’Regan and Saroj K. Nayak",
}

@article{stabilityPaper,
author = {Ataca, C. and Şahin, H. and Ciraci, S.},
title = {Stable, Single-Layer MX2 Transition-Metal Oxides and Dichalcogenides in a Honeycomb-Like Structure},
journal = {J. Phys. Chem. C},
volume = {116},
number = {16},
pages = {8983},
year = {2012},
doi = {10.1021/jp212558p},
}

@Article{Zr_Field,
author ="Kumar, Ashok and He, Haiying and Pandey, Ravindra and Ahluwalia, P. K. and Tankeshwar, K.",
title  ="Pressure and electric field-induced metallization in the phase-engineered ZrX2 (X = S{,} Se{,} Te) bilayers",
journal  ="Phys. Chem. Chem. Phys.",
year  ="2015",
volume  ="17",
issue  ="29",
pages  ="19215-19221",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C5CP01445J",
}


%@article{Vanadium,
%   author = "Wasey, A. H. M. Abdul and Chakrabarty, Soubhik and Das, G. P.",
%   title = "Quantum size effects in layered VX2 (X = S, Se) materials: Manifestation of metal to semimetal or semiconductor transition",
%   journal = "Journal of Applied Physics",
%   year = "2015",
%   volume = "117",
%   number = "6", 
%   eid = 064313,
%   pages = "",
%   doi = "http://dx.doi.org/10.1063/1.4908114" 
%}

%@article{PlatinumOx,
%  title = {Density functional theory study of platinum oxides: From infinite crystals to nanoscopic particles},
%  author = {Seriani, N. and Jin, Z. and Pompe, W. and Ciacchi, L. Colombi},
%  journal = {Phys. Rev. B},
%  volume = {76},
%  issue = {15},
%  pages = {155421},
%  numpages = {10},
%  year = {2007},
%  month = {Oct},
%  publisher = {American Physical Society},
%  doi = {10.1103/PhysRevB.76.155421},
%}


%@article{RoheniumML,
%  title = {Monolayer behaviour in bulk ReS2 due to electronic and vibrational decoupling},
%  author = {Tongay, Sefaattin and Sahin, Hasan and Ko, Changhyun and Luce, Alex and Fan, Wen and Liu, Kai and Zhou, Jian and Huang, Ying-Sheng and Ho, Ching-Hwa and Yan, Jinyuan and Ogletree, D. Frank and Aloni, Shaul and Ji, Jie and Li, Shushen and Li, Jingbo and Peeters, F. M. and Wu, Junqiao},
%  journal = {Nature Communications},
%  volume = {5},
%  pages = {3252},
%  year = {2014},
%  month = {02},
%  publisher = {Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved. SN  -},
%  url = {http://dx.doi.org/10.1038/ncomms4252}
%}


@article{Scandium,
title = "Stable ScS2 nanostructures with tunable electronic and magnetic properties ",
journal = "Solid State Commun.",
volume = "220",
number = "",
pages = "12",
year = "2015",
note = "",
issn = "0038-1098",
doi = "http://dx.doi.org/10.1016/j.ssc.2015.06.022",
author = "Hui Zhang and Xinyue Lin and Zhen-Kun Tang",

}


@Article{ScO2,
author ="Loh, G. C. and Pandey, Ravindra",
title  ="Versatile electronic properties of atomically layered ScO2",
journal  ="J. Mater. Chem. C",
year  ="2015",
volume  ="3",
issue  ="26",
pages  ="6627",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C5TC01096A",
}


@article{ScO2_ML,
  author={Hui Zhang and Chuan-Jia Tong and Jian Wu and Wen-Jin Yin and Yan-Ning Zhang},
  title={Low-dimensional ScO 2 with tunable electronic and magnetic properties: first-principles studies},
  journal={J. Phys.: Condens. Matter},
  volume={28},
  number={1},
  pages={015004},
  url={http://stacks.iop.org/0953-8984/28/i=1/a=015004},
  year={2016},
  
}
	

@article{LayeredTMDC,
title = "Electronic properties of transition-metal dichalcogenides",
doi = "10.1557/mrs.2015.143",
publisher = "Cambridge University Press",
address = "New York, USA",
author = "Agnieszka Kuc and Thomas Heine and Andras Kis",
volume = "40",
number = "7",
pages = "577-584",
year = "2015",
month = "007",
day = "001",
url = "https://www.cambridge.org/core/article/electronic-properties-of-transition-metal-dichalcogenides/0DEEE724FD103C9BD90E060F406EC4C2",
journal = "MRS Bulletin"
}


@article{ChemTMDC,
title = "The chemistry of two-dimensional layered transition metal dichalcogenide nanosheets",
publisher = "Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved",
author = "Chhowalla, Manish and Shin, Hyeon Suk and Eda, Goki and Li, Lain-Jong and Loh, Kian Ping and Zhang, Hua",
volume = "5",
number = "4",
pages = "563",
year = "2013",
month = "04",
url = "http://dx.doi.org/10.1038/nchem.1589",
journal = "Nat Chem"
}


@article{WSe2BL_field,
title = "Zeeman-type spin splitting controlled by an electric field",
publisher = "Nature Publishing Group",
author = "Yuan, Hongtao and Bahramy, Mohammad Saeed and Morimoto, Kazuhiro and Wu, Sanfeng and Nomura, Kentaro and Yang, Bohm-Jung and Shimotani, Hidekazu and Suzuki, Ryuji and Toh, Minglin and Kloc, Christian and Xu, Xiaodong and Arita, Ryotaro and Nagaosa, Naoto and Iwasa, Yoshihiro",
volume = "9",
number = "9",
pages = "563",
year = "2013",
month = "09",
url = "http://dx.doi.org/10.1038/nphys2691",
journal = "Nat. Phys."
}

%@article{WS2_bulkML,
%  title = {Electronic band structure of single-crystal and single-layer ${\mathrm{WS}}_{2}:$ Influence of interlayer van der Waals interactions},
%  author = {Klein, A. and Tiefenbacher, S. and Eyert, V. and Pettenkofer, C. and Jaegermann, W.},
%  journal = {Phys. Rev. B},
%  volume = {64},
%  issue = {20},
%  pages = {205416},
%  numpages = {14},
%  year = {2001},
%  month = {Nov},
%  publisher = {American Physical Society},
%  doi = {10.1103/PhysRevB.64.205416},
%  url = {http://link.aps.org/doi/10.1103/PhysRevB.64.205416}
%}

%@article{MoS2Se2Te2_bulk,
%  title = {Band structure of ${\mathrm{MoS}}_{2},$ ${\mathrm{MoSe}}_{2},$ and $\ensuremath{\alpha}-{\mathrm{MoTe}}_{2}:$ Angle-resolved photoelectron spectroscopy and     \textit{ab initio}   calculations},
%  author = {B\"oker, Th. and Severin, R. and M\"uller, A. and Janowitz, C. and Manzke, R. and Vo\ss{}, D. and Kr\"uger, P. and Mazur, A. and Pollmann, J.},
%  journal = {Phys. Rev. B},
%  volume = {64},
%  issue = {23},
%  pages = {235305},
%  numpages = {11},
%  year = {2001},
%  month = {Nov},
%  publisher = {American Physical Society},
%  doi = {10.1103/PhysRevB.64.235305},
%  url = {http://link.aps.org/doi/10.1103/PhysRevB.64.235305}
%}

@article{WS2BL,
title = "Bandgap engineering of different stacking \{WS2\} bilayer under an external electric field ",
journal = "Solid State Commun.",
volume = "225",
number = "",
pages = "32 - 37",
year = "2016",
note = "",
issn = "0038-1098",
doi = "http://dx.doi.org/10.1016/j.ssc.2015.10.013",
url = "http://www.sciencedirect.com/science/article/pii/S0038109815003695",
author = "Wei Li and Tianxing Wang and Xianqi Dai and Xiaolong Wang and Caiyun Zhai and Yaqiang Ma and Shanshan Chang."
}


@article{WSe2MultiL,
   author = "Dai, Xianqi and Li, Wei and Wang, Tianxing and Wang, Xiaolong and Zhai, Caiyun",
   title = "Bandstructure modulation of two-dimensional WSe2 by electric field",
   journal = "J. Appl. Phys.",
   year = "2015",
   volume = "117",
   number = "8", 
   eid = 084310,
   pages = "084310",
   doi = "http://dx.doi.org/10.1063/1.4907315" 
}


@article{bulk_TMDC,
  title = {Two-Dimensional Materials from Data Filtering and     \textit{Ab Initio}   Calculations},
  author = {Leb\`egue, S. and Bj\"orkman, T. and Klintenberg, M. and Nieminen, R. M. and Eriksson, O.},
  journal = {Phys. Rev. X},
  volume = {3},
  issue = {3},
  pages = {031002},
  numpages = {7},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.3.031002},
  url = {http://link.aps.org/doi/10.1103/PhysRevX.3.031002}
}


%@article{TiO2,
%  title = {Electronic band structure of titanium dioxide},
%  author = {Daude, N. and Gout, C. and Jouanin, C.},
%  journal = {Phys. Rev. B},
%  volume = {15},
%  issue = {6},
%  pages = {3229--3235},
%  numpages = {0},
%  year = {1977},
%  month = {Mar},
%  publisher = {American Physical Society},
%  doi = {10.1103/PhysRevB.15.3229},
%  url = {http://link.aps.org/doi/10.1103/PhysRevB.15.3229}
%}


%@article {TiS2_Miro,
%author = {Miró, Pere and Han, Jae Hyo and Cheon, Jinwoo and Heine, Thomas},
%title = {Hexagonal Transition-Metal Chalcogenide Nanoflakes with Pronounced Lateral Quantum Confinement},
%journal = {Angewandte Chemie International Edition},
%volume = {53},
%number = {46},
%publisher = {WILEY-VCH Verlag},
%issn = {1521-3773},
%url = {http://dx.doi.org/10.1002/anie.201404704},
%doi = {10.1002/anie.201404704},
%pages = {12624--12628},
%keywords = {2D materials, density functional theory, nanoflakes, quantum confinement, transition-metal chalcogenide},
%year = {2014},
%}

%@article{TiO22014,
%author = {Zhu, Tong and Gao, Shang-Peng}
%title = {The Stability, Electronic Structure, and Optical Property of TiO2 Polymorphs},
%journal = {The Journal of Physical Chemistry C},
%volume = {118},
%number = {21},
%pages = {11385-11396},
%year = {2014},
%doi = {10.1021/jp412462m},
%
%URL = { 
%        http://dx.doi.org/10.1021/jp412462m
%    
%},
%eprint = { 
%        http://dx.doi.org/10.1021/jp412462m
%    
%}
%
%}


@article {WS2Se2MyRef,
author = {W. J. Schutte, J. L. De Boer, and F. Jellinek},
title = {Crystal structures of Tungsten disulphide and diselenide},
journal = {J of Solid State Chemistry},
volume = {70},
issn = {1521-3773},
doi = {10.1016/0022-4596(87)90057-0},
pages = {207--209},
year = {1987},
}

@article{MoSe2MyRef,
author = "James, P. B. and Lavik, M. T.",
title = "{The crystal structure of MoSe${\sb 2}$}",
journal = "Acta Crystallographica",
year = "1963",
volume = "16",
number = "11",
pages = "1183",
month = "Nov",
doi = {10.1107/S0365110X6300311X},
url = {https://doi.org/10.1107/S0365110X6300311X},
}

@article{MoTe2MyRef,
author = "Puotinen, D. and Newnham, R. E.",
title = "{The crystal structure of MoTe${\sb 2}$}",
journal = "Acta Crystallographica",
year = "1961",
volume = "14",
number = "6",
pages = "691--692",
month = "Jun",
doi = {10.1107/S0365110X61002084},
url = {https://doi.org/10.1107/S0365110X61002084},
}

@article{MoS2MyRef,
author = {Dickinson, Roscoe G and Pauling, Linus},
doi = {10.1021/ja01659a020},
file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/MoS2{\_}parameters.pdf:pdf},
isbn = {0002-7863},
issn = {0002-7863},
journal = {J. Am. Chem. Soc.},
number = {6},
pages = {1466--1471},
title = {{The crystal structure of molybdenite}},
url = {http://pubs.acs.org/doi/abs/10.1021/ja01659a020},
volume = {45},
year = {1923}
}


@manual{Dovesi2013,
author = {Dovesi, R and Saunders, V R and Roetti, C and Orlando, R and Pascale, F and Civalleri, B and Doll, K and Harrison, N M and Bush, I J and Llunell, M and Science, Computational and Technologies, Advanced},
doi = {10.1524/zkri.220.5.571.65065},
pages = {1--307},
title = {{Crystal09 User's Manual}},
year = {2013},
edition={2.0.1},
organization={University of Torino: Torino},
month={February}
}

@article{dovesi2005crystal,
  title={CRYSTAL: a computational tool for the ab initio study of the electronic properties of crystals},
  author={Dovesi, Roberto and Orlando, Roberto and Civalleri, Bartolomeo and Roetti, Carla and Saunders, Victor R and Zicovich-Wilson, Claudio M},
  journal={Zeitschrift f{\"u}r Kristallographie},
  volume={220},
  number={5/6/2005},
  pages={571--573},
  year={2005}
}

@article{Dickinson1923,
author = {Dickinson, Roscoe G and Pauling, Linus},
doi = {10.1021/ja01659a020},
file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/MoS2{\_}parameters.pdf:pdf},
isbn = {0002-7863},
issn = {0002-7863},
journal = {J. Am. Chem. Soc.},
number = {6},
pages = {1466--1471},
title = {{The crystal structure of molybdenite}},
url = {http://pubs.acs.org/doi/abs/10.1021/ja01659a020},
volume = {45},
year = {1923}
}

@article{Perdew2008,
author = {Perdew, John P. and Ruzsinszky, Adrienn and Csonka, G{\'{a}}bor I. and Vydrov, Oleg A. and Scuseria, Gustavo E. and Constantin, Lucian A. and Zhou, Xiaolan and Burke, Kieron},
doi = {10.1103/PhysRevLett.100.136406},
file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/PBEsol.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
number = {13},
pages = {136406},
title = {{Restoring the Density-Gradient Expansion for Exchange in Solids and Surfaces}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.100.136406},
volume = {100},
year = {2008}
}

@article{cora1997anab,
  title={Anab initio Hartree--Fock study of $\alpha$-MoO 3},
  author={Cor{\`a}, Furio and Patel, Atul and Harrison, Nicholas M and Roetti, Carla and Catlow, C Richard A},
  journal={J. Mater. Chem.},
  volume={7},
  number={6},
  pages={959--967},
  year={1997},
  publisher={Royal Society of Chemistry}
}

%@article{Ehlers1993,
%author = {Ehlers, A.W. and B{\"{o}}hme, M. and Dapprich, S. and Gobbi, A. and H{\"{o}}llwarth, A. and Jonas, V. and K{\"{o}}hler, K.F. and Stegmann, R. and Veldkamp, A. and Frenking, G.},
%doi = {10.1016/0009-2614(93)80086-5},
%file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/HaysWadt.pdf:pdf},
%isbn = {0009-2614},
%issn = {00092614},
%journal = {Chem. Phys. Lett.},
%number = {1},
%pages = {111},
%title = {{A set of f-polarization functions for pseudo-potential basis sets of the transition metals Sc-Cu, Y-Ag and La-Au}},
%volume = {208},
%year = {1993}
%}

@article{Peintinger2013,
author = {Peintinger, Michael F. and Oliveira, Daniel Vilela and Bredow, Thomas},
doi = {10.1002/jcc.23153},
file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/S{\_}basis set.pdf:pdf},
isbn = {2379245641100},
issn = {01928651},
journal = {J. Comput. Chem.},
keywords = {CRYSTAL,TZVP,basis sets,solid-state calculations},
number = {6},
pages = {451--459},
pmid = {23115105},
title = {{Consistent Gaussian basis sets of triple-zeta valence with polarization quality for solid-state calculations}},
volume = {34},
year = {2013}
}

@article{Monkhorst1976,
author = {Monkhorst, Hendrik J. and Pack, James D.},
doi = {10.1103/PhysRevB.13.5188},
file = {:H$\backslash$:/UpdatedWork/papers-2016-01-26/papers/Monkhorst.pdf:pdf},
isbn = {0556-2805},
issn = {0556-2805},
journal = {Phys. Rev. B},
number = {12},
pages = {5188--5192},
pmid = {1966486},
title = {{Special points for Brillouin-zone integrations}},
url = {http://link.aps.org/doi/10.1103/PhysRevB.13.5188},
volume = {13},
year = {1976}
}

%@article{FSZ2016,
%author = {Xiaofeng Fan and David J. Singh and Weitao Zheng},
%title = {Valence Band Splitting on Multilayer MoS2: Mixing of Spin–Orbit Coupling and Interlayer Coupling},
%journal = {J. Phys. Chem. Lett.},
%volume = {7},
%number = {12},
%pages = {2175-2181},
%year = {2016},
%doi = {10.1021/acs.jpclett.6b00693},
%    
%URL = { 
%        http://dx.doi.org/10.1021/acs.jpclett.6b00693
%    
%},
%}

%@article{SOC2016,
%author = {Xiuming Dou and Kun Ding and Desheng Jiang and Xiaofeng Fan and Baoquan Sun},
%title = {Probing Spin–Orbit Coupling and Interlayer Coupling in Atomically Thin Molybdenum Disulfide Using Hydrostatic Pressure},
%journal = {ACS Nano},
%volume = {10},
%number = {1},
%pages = {1619-1624},
%year = {2016},
%doi = {10.1021/acsnano.5b07273},
%    
%URL = { 
%        http://dx.doi.org/10.1021/acsnano.5b07273
%    
%},
%
%}



@article {NiPdPtX2BL,
author = {Miró, Pere and Ghorbani-Asl, Mahdi and Heine, Thomas},
title = {Two Dimensional Materials Beyond MoS2: Noble-Transition-Metal Dichalcogenides},
journal = {Angew. Chem. Int. Ed.},
volume = {53},
number = {11},
publisher = {WILEY-VCH Verlag},
issn = {1521-3773},
url = {http://dx.doi.org/10.1002/anie.201309280},
doi = {10.1002/anie.201309280},
pages = {3015-3018},
keywords = {2D materials, chalcogenides, noble metals, palladium, platinum},
year = {2014},
}


@article{SET,
  author={M Javaid and Daniel W Drumm and Salvy P Russo and Andrew D Greentree},
  title={Surface-gate-defined single-electron transistor in a MoS 2 bilayer},
  journal={Nanotechnology},
  volume={28},
  number={12},
  pages={125203},
  url={http://stacks.iop.org/0957-4484/28/i=12/a=125203},
  year={2017},

}


@article{Novoselove,
title = "Two-dimensional gas of massless {Dirac} fermions in graphene",
journal = "Nature",
volume = "438",
number = "7065",
pages = "197-200",
year = "2005",
author = "Novoselov, K. S. and Geim, A. K. and Morozov, S. V. and Jiang, D. and Katsnelson, M. I. and Grigorieva, I. V. and Dubonos, S. V. and Firsov, A. A.",
}

@article{TMDCs_photonics,
title = "Photonics and optoelectronics of 2{D} semiconductor transition metal dichalcogenides",
journal = "Nat. Photon",
volume = "10",
number = "4",
pages = "216-226",
year = "2016",
author = "Mak, Kin Fai and Shan, Jie",
}


@Article{GeneralFormula,
author ="Wang, Qing Hua and Kalantar-Zadeh, Kourosh and Kis, Andras and Coleman, Jonathan N. and Strano, Michael S.",
title  ="Electronics and optoelectronics of two-dimensional transition metal dichalcogenides",
journal  ="Nat. Nanotechnol.",
year  ="2012",
volume  ="7",
number = "11",
issue  ="",
pages  ="699-712",
publisher  ="Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved."
}

@article{XLF2012,
  title = {Coupled Spin and Valley Physics in Monolayers of {MoS$_{2}$} and Other Group-{VI} Dichalcogenides},
  author = {Xiao, Di and Liu, Gui-Bin and Feng, Wanxiang and Xu, Xiaodong and Yao, Wang},
  journal = {Phys. Rev. Lett.},
  volume = {108},
  issue = {19},
  pages = {196802},
  numpages = {5},
  year = {2012},
  month = {May},
  publisher = {American Physical Society},
}


@article {Grimme,
author = {Grimme, Stefan},
title = {Semiempirical GGA-type density functional constructed with a long-range dispersion correction},
journal = {J. Comput. Chem.},
volume = {27},
number = {15},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1096-987X},
doi = {10.1002/jcc.20495},
pages = {1787},
year = {2006},
}




%@article{T-TiS2Structure,
%
%title = {Electronic structure of TiS2 and its electric transport properties under high pressure},
%author={Bao Liu. Jie Yang, Yonghao Han, Tingjing Hu, Wanbin Ren, Cailong Liu, Yanzhang Ma, and and Chunxiao Gao},
%journal = {Journal of Applied Physics},
%volume = {109},
%number = {5},
%pages = {053717},
%year = {2011},
%doi = {10.1063/1.3552299}
%}

%@article{T-TiSe2Structure,
%
%title = {The pressure dependences of Tis, and TiSe, band structures},
%author={G A Benesh, A M Woolley and C Umrigar},
%journal = {J. Phys. C: Solid State Phys.},
%volume = {18},
%number = {18},
%pages = {1595-1603},
%year = {1985},
%doi = {https://doi.org/10.1088/0022-3719/18/8/007}
%}


@article{H-TiO2Structure,
author = {Lu, Y. H. and Xu, B. and Zhang, A. H. and Yang, M. and Feng, Y. P.},
title = {Hexagonal TiO2 for Photoelectrochemical Applications},
journal = {J. Phys. Chem. C},
volume = {115},
number = {36},
pages = {18042-18045},
year = {2011},
doi = {10.1021/jp205439x}
}

@article {Sc_BS,
author = {Peintinger, Michael F. and Oliveira, Daniel Vilela and Bredow, Thomas},
title = {Consistent Gaussian basis sets of triple-zeta valence with polarization quality for solid-state calculations},
journal = {J. Comput. Chem.},
volume = {34},
number = {6},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
issn = {1096-987X},
doi = {10.1002/jcc.23153},
pages = {451-459},
year ={2013},
}

@article {Zr_BS,
author = {Bredow, Thomas and Lerch, Martin},
title = {Anion Distribution in Zr2ON2},
journal = {Zeitschrift für anorganische und allgemeine Chemie},
volume = {630},
number = {13-14},
publisher = {WILEY-VCH Verlag},
issn = {1521-3749},
url = {http://dx.doi.org/10.1002/zaac.200400166},
doi = {10.1002/zaac.200400166},
pages = {2262--2266},
keywords = {Zirconium oxynitride, DFT calculation, Anion distribution},
year = {2004},
}

@article{Hf_BS,
  title = {Spectroscopic properties of oxygen vacancies in monoclinic $\mathrm{Hf}{\mathrm{O}}_{2}$ calculated with periodic and embedded cluster density functional theory},
  author = {Mu\~noz Ramo, D. and Gavartin, J. L. and Shluger, A. L. and Bersuker, G.},
  journal = {Phys. Rev. B},
  volume = {75},
  issue = {20},
  pages = {205336},
  numpages = {12},
  year = {2007},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.75.205336},
}

@article{Mo_BS,
  title={Anab initio Hartree--Fock study of $\alpha$-MoO 3},
  author={Cor{\`a}, Furio and Patel, Atul and Harrison, Nicholas M and Roetti, Carla and Catlow, C Richard A},
  journal={J. Mater. Chem.},
  volume={7},
  number={6},
  pages={959--967},
  year={1997},
  publisher={Royal Society of Chemistry}
}

@article{W_BS,
author = {Corà, Furio and Patel, Atul and Harrison, Nicholas M. and Dovesi, Roberto and Catlow, C. Richard A.},
title = {An ab Initio Hartree−Fock Study of the Cubic and Tetragonal Phases of Bulk Tungsten Trioxide},
journal = {J. Am. Chem. Soc.},
volume = {118},
number = {48},
pages = {12174-12182},
year = {1996},
doi = {10.1021/ja961514u},
}


@article{Pd_BS,
title = "Orientation of N2O molecule on Pd(110) surface",
journal = "Surf. Sci.",
volume = "506",
number = "3",
pages = "196 - 202",
year = "2002",
note = "",
issn = "0039-6028",
doi = "http://dx.doi.org/10.1016/S0039-6028(02)01435-8",
author = "Anton Kokalj and Ivan Kobal and Hideyuki Horino and Yuichi Ohno and Tatsuo Matsushima",
}

@article{Pt_BS,
title = "CO adsorption on the Pt(111) surface: a comparison of a gradient corrected functional and a hybrid functional",
journal = "Surf. Sci.",
volume = "573",
number = "3",
pages = "464 - 473",
year = "2004",
issn = "0039-6028",
doi = "http://dx.doi.org/10.1016/j.susc.2004.10.015",
author = "K. Doll",
}

@article{Te_BS,
author = {Jochen Heyd and Juan E. Peralta and Gustavo E. Scuseria and Richard L. Martin},
title = {Energy band gaps and lattice parameters evaluated with the Heyd-Scuseria-Ernzerhof screened hybrid functional},
journal = {J. Chem. Phys.},
volume = {123},
number = {17},
pages = {174101},
year = {2005},
doi = {10.1063/1.2085170},
}

@article{SET_Angus,
author = {Angus, Susan J. and Ferguson, Andrew J. and Dzurak, Andrew S. and Clark, Robert G.},
title = {Gate-Defined Quantum Dots in Intrinsic Silicon},
journal = {Nano Lett.},
volume = {7},
number = {7},
pages = {2051-2055},
year = {2007},
doi = {10.1021/nl070949k},
}


@article{Wilson_1960,
author = { J.A. Wilson and A.D. Yoffe },
title = {The transition metal dichalcogenides discussion and interpretation of the observed optical, electrical and structural properties},
journal = {Adv. Phys.},
volume = {18},
number = {73},
pages = {193-335},
year = {1969},
doi = {10.1080/00018736900101307},
}

@article{TMDCReview1,
author ="Manzeli, Sajedeh and Ovchinnikov, Dmitry and Pasquier, Diego and Yazyev, Oleg V. and Kis, Andras",
title  ="2D transition metal dichalcogenides",
journal  ="Nat. Rev. Mater.",
year  ="2017",
volume  ="2",
issue  ="9",
pages  ="17033",
publisher  ="Macmillan Publishers Limited SN  -",
doi  ="10.1038/natrevmats.2017.33"
}

@article{TMDCsReview,
author ="Duan, Xidong and Wang, Chen and Pan, Anlian and Yu, Ruqin and Duan, Xiangfeng",
title  ="Two-dimensional transition metal dichalcogenides as atomically thin semiconductors: opportunities and challenges",
journal  ="Chem. Soc. Rev.",
year  ="2015",
volume  ="44",
issue  ="24",
pages  ="8859-8876",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C5CS00507H"
}



@article{T-ZrX2_ML,
author = {Guo, Hongyan and Lu, Ning and Wang, Lu and Wu, Xiaojun and Zeng, Xiao Cheng},
title = {Tuning Electronic and Magnetic Properties of Early Transition-Metal Dichalcogenides via Tensile Strain},
journal = {J. Phys. Chem. C},
volume = {118},
number = {13},
pages = {7242-7249},
year = {2014},
doi = {10.1021/jp501734s},

}


@article{watersplitting,
author = {N{\o}rskov, J. K. and Rossmeisl, J. and Logadottir, A. and Lindqvist, L. and Kitchin, J. R. and Bligaard, T. and J\'{o}nsson, H.},
title = {Origin of the Overpotential for Oxygen Reduction at a Fuel-Cell Cathode},
journal = {J. Phys. Chem. B},
volume = {108},
number = {46},
pages = {17886-17892},
month ={October},
year = {2004},
doi = {10.1021/jp047349j}
}


@article {Yeh2014,
author = {Yeh, Te-Fu and Teng, Chiao-Yi and Chen, Shean-Jen and Teng, Hsisheng},
title = {Nitrogen-Doped Graphene Oxide Quantum Dots as Photocatalysts for Overall Water-Splitting under Visible Light Illumination},
journal = {Adv. Mater.},
volume = {26},
number = {20},
issn = {1521-4095},
doi = {10.1002/adma.201305299},
pages = {3297-3303},
month= {February},
year = {2014},
}

@article{Singh2015,
author = {Singh, Arunima K. and Mathew, Kiran and Zhuang, Houlong L. and Hennig, Richard G.},
title = {Computational Screening of 2D Materials for Photocatalysis},
journal = {J. Phys. Chem. Lett.},
volume = {6},
number = {6},
pages = {1087-1098},
month ={February},
year = {2015},
doi = {10.1021/jz502646d},
}

@article{Trasatti1986,
author = {Trasatti, S.},
title = {The absolute electrode potential: an explanatory note (Recommendations 1986)},
journal = {Pure \& Appl. Chem.},
volume = {58},
number = {7},
pages = {955-966},
month ={January},
year = {1986},
doi = {10.1351/pac198658070955},
}

@article{Butler1978,
author = {Butler, M. A. and Ginley, D. S.}, 
title = {Prediction of Flatband Potentials at Semiconductor‐Electrolyte Interfaces from Atomic Electronegativities},
volume = {125}, 
number = {2}, 
pages = {228-232}, 
month ={February},
year = {1978}, 
doi = {10.1149/1.2131419}, 
journal = {J. Electrochem. Soc.} 
}



@article{Phosphorus,
author = {Liu, Yanpeng and Qiu, Zhizhan and Carvalho, Alexandra and Bao, Yang and Xu, Hai and Tan, Sherman J. R. and Liu, Wei and Castro Neto, A. H. and Loh, Kian Ping and Lu, Jiong},
title = {{Gate-Tunable Giant Stark Effect in Few-Layer Black Phosphorus}},
journal = {Nano Lett.},
volume = {17},
number = {3},
pages = {1970-1977},
month={February},
year = {2017},
doi = {10.1021/acs.nanolett.6b05381},
URL = { 
        http://dx.doi.org/10.1021/acs.nanolett.6b05381   
},
}



@article{Graphene_Field,
  title = {Observation of an Electric-Field-Induced Band Gap in Bilayer Graphene by Infrared Spectroscopy},
  author = {Mak, Kin Fai and Lui, Chun Hung and Shan, Jie and Heinz, Tony F.},
  journal = {Phys. Rev. Lett.},
  volume = {102},
  issue = {25},
  pages = {256405 (1-4)},
  numpages = {4},
  year = {2009},
  month = {June},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.102.256405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.102.256405}
}


@article{Graphene_field2,
author={Zhang,Yuanbo and Tang,Tsung-Ta and Girit,Caglar and Hao,Zhao and Martin,Michael C. and Zettl,Alex and Crommie,Michael F. and Shen,Y. R. and Wang,Feng},
year={2009},
month={June},
title={Direct observation of a widely tunable bandgap in bilayer graphene},
journal={Nature},
volume={459},
number={7248},
pages={820-823},
isbn={00280836},
doi ={10.1038/nature08105}
}

@article{BG_Field,
author = {Ni, Zeyuan and Liu, Qihang and Tang, Kechao and Zheng, Jiaxin and Zhou, Jing and Qin, Rui and Gao, Zhengxiang and Yu, Dapeng and Lu, Jing},
title = {Tunable Bandgap in Silicene and Germanene},
journal = {Nano Lett.},
volume = {12},
number = {1},
pages = {113-118},
year = {2012},
month =[november},
doi = {10.1021/nl203065e},

}



@article{CN_Field,
  author={Chun-Wei Chen and Ming-Hsien Lee and S J Clark},
  title={Band gap modification of single-walled carbon nanotube and boron nitride nanotube under a transverse electric field},
  journal={Nanotechnology},
  volume={15},
  number={12},
  month ={November},
  pages={1837-1843},
  url={http://stacks.iop.org/0957-4484/15/i=12/a=025},
  year={2004},
 
}

%@book{Book,
%Title={Physics of Semiconductor Devices},
%Authors	={Simon M. Sze, Kwok K. Ng},
%Publisher={	John Wiley & Sons},
%edition ={3},
%ISBN	 ={0470068302},
%year ={2006}
%}


@book{Wiley,
author = {Simon M. Sze, Kwok K. Ng},
isbn = {0470068302},
year ={2006},
publisher = {John Wiley \& Sons},
title = {{Physics of Semiconductor Devices, Edition 3}},
}


@article{2DMat5,
author = {Wang, Han and Yu, Lili and Lee, Yi-Hsien and Shi, Yumeng and Hsu, Allen and Chin, Matthew L. and Li, Lain-Jong and Dubey, Madan and Kong, Jing and Palacios, Tomas},
title = {Integrated Circuits Based on Bilayer MoS2 Transistors},
journal = {Nano Lett.},
volume = {12},
number = {9},
pages = {4674-4680},
year = {2012},
doi = {10.1021/nl302015v},

}


@article{2DMat1,
author = {Akinwande, Deji and Petrone, Nicholas and Hone, James},
journal = {Nat. Commun.},
pages = {5678},
title = {{Two-dimensional flexible nanoelectronics}},
volume = {5},
year = {2014}
}


@article{2DMat4,
  author={Xiaofeng Qian and Yangyang Wang and Wenbin Li and Jing Lu and Ju Li},
  title={Modelling of stacked 2D materials and devices},
  journal={2D Mater.},
  volume={2},
  number={3},
  pages={032003},
  url={http://stacks.iop.org/2053-1583/2/i=3/a=032003},
  year={2015}
}

@article{Geim,
author ="Geim, A. K. and Novoselov, K. S.",
title  ="The rise of graphene",
journal  ="Nat. Mater.",
year  ="2007",
volume  ="6",
number = "3",
pages  ="183-191",
url  ="http://dx.doi.org/10.1038/nmat1849"
}


@Article{Ning2014,
author ="Lu, Ning and Guo, Hongyan and Li, Lei and Dai, Jun and Wang, Lu and Mei, Wai-Ning and Wu, Xiaojun and Zeng, Xiao Cheng",
title  ="MoS2/MX2 heterobilayers: bandgap engineering via tensile strain or external electrical field",
journal  ="Nanoscale",
year  ="2014",
volume  ="6",
issue  ="5",
pages  ="2879-2886",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C3NR06072A",
}

@article{Dongwei,
  author={Dongwei Xu and Haiying He and Ravindra Pandey and Shashi P Karna},
  title={Stacking and electric field effects in atomically thin layers of GaN},
  journal={J. Phys.: Condens. Matter},
  volume={25},
  number={34},
  pages={345302},
  url={http://stacks.iop.org/0953-8984/25/i=34/a=345302},
  year={2013},
}

@article{Balu2012,
author = {Radhakrishnan Balu and Xiaoliang Zhong and Ravindra Pandey and Shashi P. Karna},
title = {Effect of electric field on the band structure of graphene/boron nitride and boron nitride/boron nitride bilayers},
journal = {Appl. Phys. Lett.},
volume = {100},
number = {5},
pages = {052104},
year = {2012},
doi = {10.1063/1.3679174},
}

@article{Golberg2010,
author = {Golberg, Dmitri and Bando, Yoshio and Huang, Yang and Terao, Takeshi and Mitome, Masanori and Tang, Chengchun and Zhi, Chunyi},
title = {Boron Nitride Nanotubes and Nanosheets},
journal = {ACS Nano},
volume = {4},
number = {6},
pages = {2979-2993},
year = {2010},
doi = {10.1021/nn1006495},

}


@Article{Osada2009,
author ="Osada, Minoru and Sasaki, Takayoshi",
title  ="Exfoliated oxide nanosheets: new solution to nanoelectronics",
journal  ="J. Mater. Chem.",
year  ="2009",
volume  ="19",
issue  ="17",
pages  ="2503-2511",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/B820160A",
}


@article{Hongqi_1,
  title = {Asymmetric nonlinear conductance of quantum dots with broken inversion symmetry},
  author = {Linke, H. and Sheng, W. D. and Svensson, A. and L\"ofgren, A. and Christensson, L. and Xu, H. Q. and Omling, P. and Lindelof, P. E.},
  journal = {Phys. Rev. B},
  volume = {61},
  issue = {23},
  pages = {15914-15926},
  numpages = {0},
  year = {2000},
  month = {June},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.61.15914},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.61.15914}
}

@article{Hongqi_2,
author = {Jie Sun and Marcus Larsson and Ivan Maximov and Hilde Hardtdegen and H. Q. Xu},
title = {Gate-defined quantum-dot devices realized in InGaAs/InP by incorporating a HfO2 layer as gate dielectric},
journal = {Appl. Phys. Lett.},
volume = {94},
number = {4},
month ={January},
pages = {042114},
year = {2009},
doi = {10.1063/1.3077188},
}


